A Note on the Estimation of Job Amenities and Labor Productivity

This paper introduces a maximum likelihood estimator of the value of job amenities and labor productivity in a single matching market based on the observation of equilibrium matches and wages. The estimation procedure simultaneously fits both the matching patterns and the wage curve. While our estimator is suited for a wide range of assignment problems, we provide an application to the estimation of the Value of a Statistical Life using compensating wage differentials for the risk of fatal injury on the job. Using US data for 2017, we estimate the Value of Statistical Life at \$ 6.3 million (\$2017).

==> Outputs/AffinityTab.tex <==
 Job Amenities (Alpha) &Risk (in 100,000) &     Public                   \\ 
YoS (in years)        &   0.09 &  & (  0.03) & (Experience (in years) &   0.00 &  & (  0.02) & (Female                &   0.18 &  & (  0.07) & (

==> Outputs/AffinityTab10.tex <==
 Job Amenities (Alpha) &Risk (in 100,000) &     Public                   \\ 
YoS (in years) &  &   0.09 \\ 
 & () & (  0.03) \\ 
Union Member   &  &   0.18 \\ 
 & () & (  0.07) \\ 
\hline  Productivity (Gamma) &Risk (in 100,000) &    Public                  \\ 
YoS (in years)        &  -0.04 &   0.35 \\ 
 & (  0.01) & (  0.05) \\ 
Experience (in years) &   0.03 &   0.05 \\ 
 & (  0.01) & (  0.04) \\ 
Female                &  -1.01 &   0.21 \\ 
 & (  0.10) & (  0.09) \\ 
Union Member          &   0.02 &   1.26 \\ 
 & (  0.05) & (  0.12) \\ 
\hline\hline 


==> Outputs/AffinityTab15.tex <==
 Job Amenities (Alpha) &Risk (in 100,000) &     Public                   \\ 
YoS (in years)        &   0.00 &   0.10 \\ 
 & (  0.01) & (  0.04) \\ 
Experience (in years) &  -0.00 &   0.00 \\ 
 & (  0.01) & (  0.02) \\ 
Female                &  -0.05 &   0.05 \\ 
 & (  0.05) & (  0.04) \\ 
Union Member          &  -0.01 &   0.24 \\ 
 & (  0.02) & (  0.10) \\ 
\hline  Productivity (Gamma) &Risk (in 100,000) &    Public                  \\ 
YoS (in years)        &  -0.04 &   0.35 \\ 
 & (  0.01) & (  0.05) \\ 
Experience (in years) &   0.03 &   0.05 \\ 
 & (  0.02) & (  0.04) \\ 
Female                &  -0.99 &   0.20 \\ 
 & (  0.12) & (  0.09) \\ 
Union Member          &   0.02 &   1.25 \\ 
 & (  0.05) & (  0.13) \\ 
\hline\hline 


==> Outputs/AffinityTab_QE10.tex <==
 Job Amenities (Alpha) &Risk (in 100,000) &     Public                   \\ 
YoS (in years) &  &   0.08 \\ 
 & () & (  0.03) \\ 
\hline  Productivity (Gamma) &Risk (in 100,000) &    Public                  \\ 
YoS (in years)        &  -0.06 &   0.84 \\ 
 & (  0.02) & (  0.10) \\ 
Experience (in years) &   0.07 &   0.10 \\ 
 & (  0.03) & (  0.10) \\ 
Female                &  -2.39 &   0.55 \\ 
 & (  0.24) & (  0.21) \\ 
\hline\hline 


==> Outputs/AffinityTab_QE12.tex <==
 Job Amenities (Alpha) &Risk (in 100,000) &     Public                   \\ 
YoS (in years) &  &   0.08 \\ 
 & () & (  0.03) \\ 
\hline  Productivity (Gamma) &Risk (in 100,000) &    Public                  \\ 
YoS (in years)        &  -0.00 &  -0.06 \\ 
 & (  0.00) & (  0.03) \\ 
Experience (in years) &   0.00 &   0.01 \\ 
 & (  0.00) & (  0.00) \\ 
Female                &  -0.05 &   0.01 \\ 
 & (  0.01) & (  0.01) \\ 
\hline\hline 


==> Outputs/AffinityTab_QE15.tex <==
 Job Amenities (Alpha) &Risk (in 100,000) &     Public                   \\ 
YoS (in years)        &   0.00 &   0.11 \\ 
 & (  0.01) & (  0.04) \\ 
Experience (in years) &  -0.00 &   0.02 \\ 
 & (  0.01) & (  0.02) \\ 
Female                &  -0.07 &   0.02 \\ 
 & (  0.03) & (  0.04) \\ 
\hline  Productivity (Gamma) &Risk (in 100,000) &    Public                  \\ 
YoS (in years)        &  -0.01 &  -0.06 \\ 
 & (  0.01) & (  0.04) \\ 
Experience (in years) &   0.01 &   0.00 \\ 
 & (  0.01) & (  0.02) \\ 
Female                &  -0.04 &   0.00 \\ 
 & (  0.03) & (  0.04) \\ 
\hline\hline 


==> Outputs/AffinityTab_QE16.tex <==
 Job Amenities (Alpha) &Risk (in 100,000) &     Public                   \\ 
YoS (in years)        &  -0.00 &   0.10 \\ 
 & (  0.01) & (  0.04) \\ 
Experience (in years) &   0.00 &  -0.00 \\ 
 & (  0.01) & (  0.02) \\ 
Female                &  -0.05 &   0.04 \\ 
 & (  0.06) & (  0.04) \\ 
\hline  Productivity (Gamma) &Risk (in 100,000) &    Public                  \\ 
YoS (in years)        &  -0.06 &   0.85 \\ 
 & (  0.02) & (  0.10) \\ 
Experience (in years) &   0.07 &   0.10 \\ 
 & (  0.03) & (  0.10) \\ 
Female                &  -2.39 &   0.55 \\ 
 & (  0.25) & (  0.21) \\ 
\hline\hline 


==> Outputs/Coef_Risk.tex <==
  2.53

==> Outputs/Coef_Risk10.tex <==
  2.47

==> Outputs/Coef_Risk11.tex <==
  2.53

==> Outputs/Coef_Risk15.tex <==
  1.79

==> Outputs/Coef_Risk_QE.tex <==
-45.97

==> Outputs/Coef_Risk_QE11.tex <==
-54.82

==> Outputs/Coef_Risk_QE12.tex <==
  2.44

==> Outputs/Coef_Risk_QE15.tex <==
  1.65

==> Outputs/Coef_Risk_QE16.tex <==
  1.65

==> Outputs/Coef_Risk_fem.tex <==
 -0.16

==> Outputs/Coef_Risk_fem15.tex <==
  6.63

==> Outputs/Coef_Risk_fem_QE15.tex <==
  7.05

==> Outputs/Coef_Risk_fem_QE16.tex <==
  7.05

==> Outputs/MainEffectsTab.tex <==
 Job Amenities (Alpha) &&                       Risk (in 100,000) &     Public                   \\ 
Main effects          &  &  -0.02 &  -0.05 \\ 
 &  & (  0.01) & (  0.03) \\ 
\hline  Productivity (Gamma) & Main effects &  &  \\  
YoS (in years)        &   0.12 &  &  \\ 
 & (  0.04) &  &  \\ 
Experience (in years) &   0.08 &  &  \\ 
 & (  0.02) &  &  \\ 
Female                &  -0.25 &  &  \\ 
 & (  0.04) &  &  \\ 
Married               &   0.07 &  &  \\ 
 & (  0.02) &  &  \\ 
Union Member          &  -0.01 &  &  \\ 
 & (  0.07) &  &  \\ 
White                 &   0.03 &  &  \\ 
 & (  0.02) &  &  \\ 
Black                 &  -0.12 &  &  \\ 
 & (  0.04) &  &  \\ 
Asian                 &   0.07 &  &  \\ 
 & (  0.03) &  &  \\ 
\hline Salary constant &   2.81 &  &  \\ 
 & (  0.15) &  &  \\ 
\hline\hline 


==> Outputs/MainEffectsTab10.tex <==
 Job Amenities (Alpha) &&                       Risk (in 100,000) &     Public                   \\ 
Main effects          &  &  -0.02 &  -0.05 \\ 
 &  & (  0.01) & (  0.03) \\ 
\hline  Productivity (Gamma) & Main effects &  &  \\  
YoS (in years)        &   0.12 &  &  \\ 
 & (  0.04) &  &  \\ 
Experience (in years) &   0.08 &  &  \\ 
 & (  0.02) &  &  \\ 
Female                &  -0.25 &  &  \\ 
 & (  0.04) &  &  \\ 
Married               &   0.07 &  &  \\ 
 & (  0.02) &  &  \\ 
Union Member          &  -0.01 &  &  \\ 
 & (  0.07) &  &  \\ 
White                 &   0.03 &  &  \\ 
 & (  0.02) &  &  \\ 
Black                 &  -0.12 &  &  \\ 
 & (  0.04) &  &  \\ 
Asian                 &   0.07 &  &  \\ 
 & (  0.03) &  &  \\ 
\hline Salary constant &   2.81 &  &  \\ 
 & (  0.15) &  &  \\ 
Sigma 1 &   0.04 &  &  \\ 
Sigma 2 &   0.92 &  &  \\ 
\hline R-square &  0.242 &  &  \\ 
\hline\hline 


==> Outputs/MainEffectsTab11.tex <==
 Job Amenities (Alpha) &&                       Risk (in 100,000) &     Public                   \\ 
Main effects          &  &  -0.03 &   0.01 \\ 
 &  & (  0.01) & (  0.02) \\ 
\hline  Productivity (Gamma) & Main effects &  &  \\  
YoS (in years)        &   0.15 &  &  \\ 
 & (  0.02) &  &  \\ 
Experience (in years) &   0.08 &  &  \\ 
 & (  0.01) &  &  \\ 
Female                &  -0.14 &  &  \\ 
 & (  0.02) &  &  \\ 
Married               &   0.07 &  &  \\ 
 & (  0.02) &  &  \\ 
Union Member          &   0.22 &  &  \\ 
 & (  0.04) &  &  \\ 
White                 &   0.03 &  &  \\ 
 & (  0.02) &  &  \\ 
Black                 &  -0.13 &  &  \\ 
 & (  0.02) &  &  \\ 
Asian                 &   0.06 &  &  \\ 
 & (  0.03) &  &  \\ 
\hline Salary constant &   0.34 &  &  \\ 
 & (  0.00) &  &  \\ 
Sigma 1 &   0.06 &  &  \\ 
Sigma 2 &   0.06 &  &  \\ 
\hline R-square &  0.235 &  &  \\ 
\hline\hline 


==> Outputs/MainEffectsTab15.tex <==
 Job Amenities (Alpha) &&                       Risk (in 100,000) &     Public                   \\ 
Main effects          &  &  -0.02 &  -0.08 \\ 
 &  & (  0.01) & (  0.04) \\ 
\hline  Productivity (Gamma) & Main effects &  &  \\  
YoS (in years)        &   0.12 &  &  \\ 
 & (  0.04) &  &  \\ 
Experience (in years) &   0.08 &  &  \\ 
 & (  0.02) &  &  \\ 
Female                &  -0.24 &  &  \\ 
 & (  0.04) &  &  \\ 
Married               &   0.07 &  &  \\ 
 & (  0.02) &  &  \\ 
Union Member          &  -0.01 &  &  \\ 
 & (  0.07) &  &  \\ 
White                 &   0.03 &  &  \\ 
 & (  0.02) &  &  \\ 
Black                 &  -0.12 &  &  \\ 
 & (  0.04) &  &  \\ 
Asian                 &   0.07 &  &  \\ 
 & (  0.03) &  &  \\ 
\hline Salary constant &   3.20 &  &  \\ 
 & (  0.43) &  &  \\ 
Sigma 1 &   0.08 &  &  \\ 
Sigma 2 &   0.91 &  &  \\ 
\hline R-square &  0.245 &  &  \\ 
\hline\hline 


==> Outputs/MainEffectsTab_QE11.tex <==
 Job Amenities (Alpha) &&                       Risk (in 100,000) &     Public                   \\ 
Main effects                  &  &   0.55 &   0.63 \\ 
 &  & (  0.03) & (  0.09) \\ 
\hline  Productivity (Gamma) & Main effects &  &  \\  
YoS (in years)                &   0.83 &  &  \\ 
 & (  0.02) &  &  \\ 
Experience (in years)         &   0.75 &  &  \\ 
 & (  0.03) &  &  \\ 
Female                        &   0.50 &  &  \\ 
 & (  0.06) &  &  \\ 
Married                       &   0.51 &  &  \\ 
 & (  0.07) &  &  \\ 
White                         &   0.57 &  &  \\ 
 & (  0.08) &  &  \\ 
Black                         &   0.70 &  &  \\ 
 & (  0.12) &  &  \\ 
Asian                         &   0.68 &  &  \\ 
 & (  0.15) &  &  \\ 
YoS squared                   &   0.31 &  &  \\ 
 & (  0.04) &  &  \\ 
\hline Salary constant &   0.10 &  &  \\ 
 & (  0.00) &  &  \\ 
Sigma 1 &   3.35 &  &  \\ 
Sigma 2 &   3.35 &  &  \\ 
\hline R-square & -9.089 &  &  \\ 
\hline\hline 


==> Outputs/MainEffectsTab_QE12.tex <==
 Job Amenities (Alpha) &&                       Risk (in 100,000) &     Public                   \\ 
Main effects                  &  &  -0.02 &  -0.06 \\ 
 &  & (  0.01) & (  0.03) \\ 
\hline  Productivity (Gamma) & Main effects &  &  \\  
YoS (in years)                &   0.17 &  &  \\ 
 & (  0.07) &  &  \\ 
Experience (in years)         &   0.09 &  &  \\ 
 & (  0.04) &  &  \\ 
Female                        &  -0.15 &  &  \\ 
 & (  0.06) &  &  \\ 
Married                       &   0.05 &  &  \\ 
 & (  0.03) &  &  \\ 
White                         &   0.05 &  &  \\ 
 & (  0.02) &  &  \\ 
Black                         &  -0.11 &  &  \\ 
 & (  0.05) &  &  \\ 
Asian                         &   0.07 &  &  \\ 
 & (  0.04) &  &  \\ 
YoS squared                   &   0.02 &  &  \\ 
 & (  0.01) &  &  \\ 
Experience squared (in years) &  -0.05 &  &  \\ 
 & (  0.02) &  &  \\ 
\hline Salary constant &   3.00 &  &  \\ 
 & (  0.01) &  &  \\ 
Sigma 1 &   0.05 &  &  \\ 
Sigma 2 &   0.00 &  &  \\ 
\hline R-square &  0.234 &  &  \\ 
\hline\hline 


==> Outputs/MainEffectsTab_QE15.tex <==
 Job Amenities (Alpha) &&                       Risk (in 100,000) &     Public                   \\ 
Main effects                  &  &  -0.02 &  -0.07 \\ 
 &  & (  0.02) & (  0.04) \\ 
\hline  Productivity (Gamma) & Main effects &  &  \\  
YoS (in years)                &   0.17 &  &  \\ 
 & (  0.09) &  &  \\ 
Experience (in years)         &   0.09 &  &  \\ 
 & (  0.05) &  &  \\ 
Female                        &  -0.15 &  &  \\ 
 & (  0.08) &  &  \\ 
Married                       &   0.05 &  &  \\ 
 & (  0.03) &  &  \\ 
White                         &   0.05 &  &  \\ 
 & (  0.03) &  &  \\ 
Black                         &  -0.11 &  &  \\ 
 & (  0.06) &  &  \\ 
Asian                         &   0.07 &  &  \\ 
 & (  0.05) &  &  \\ 
YoS squared                   &   0.02 &  &  \\ 
 & (  0.01) &  &  \\ 
Experience squared (in years) &  -0.05 &  &  \\ 
 & (  0.03) &  &  \\ 
\hline Salary constant &   3.45 &  &  \\ 
 & (  0.05) &  &  \\ 
Sigma 1 &   0.00 &  &  \\ 
Sigma 2 &   6.41 &  &  \\ 
\hline R-square & -6.622 &  &  \\ 
\hline\hline 


==> Outputs/MainEffectsTab_QE16.tex <==
 Job Amenities (Alpha) &&                       Risk (in 100,000) &     Public                   \\ 
Main effects                  &  &  -0.02 &  -0.08 \\ 
 &  & (  0.01) & (  0.04) \\ 
\hline  Productivity (Gamma) & Main effects &  &  \\  
YoS (in years)                &   0.06 &  &  \\ 
 & (  0.04) &  &  \\ 
Experience (in years)         &   0.08 &  &  \\ 
 & (  0.03) &  &  \\ 
Female                        &  -0.40 &  &  \\ 
 & (  0.06) &  &  \\ 
Married                       &   0.05 &  &  \\ 
 & (  0.02) &  &  \\ 
White                         &   0.05 &  &  \\ 
 & (  0.02) &  &  \\ 
Black                         &  -0.11 &  &  \\ 
 & (  0.04) &  &  \\ 
Asian                         &   0.07 &  &  \\ 
 & (  0.04) &  &  \\ 
Experience squared (in years) &  -0.05 &  &  \\ 
 & (  0.02) &  &  \\ 
\hline Salary constant &   3.37 &  &  \\ 
 & (  1.08) &  &  \\ 
Sigma 1 &   0.09 &  &  \\ 
Sigma 2 &   2.25 &  &  \\ 
\hline R-square &  0.235 &  &  \\ 
\hline\hline 


==> Outputs/Risk.tex <==
 -0.96

==> Outputs/SDVOSL.tex <==
   2.1

==> Outputs/SDVOSL10.tex <==
   2.5

==> Outputs/SDVOSL11.tex <==
   2.1

==> Outputs/SDVOSL15.tex <==
   3.0

==> Outputs/SDVOSL_QE.tex <==
   6.5

==> Outputs/SDVOSL_QE10.tex <==
   2.5

==> Outputs/SDVOSL_QE11.tex <==
   7.2

==> Outputs/SDVOSL_QE12.tex <==
   3.3

==> Outputs/SDVOSL_QE15.tex <==
   3.1

==> Outputs/SDVOSL_QE16.tex <==
   3.1

==> Outputs/Try_figure.tex <==
 16.47 \\ 


==> Outputs/VOSL.tex <==
   7.0

==> Outputs/VOSL10.tex <==
   6.8

==> Outputs/VOSL11.tex <==
   7.0

==> Outputs/VOSL15.tex <==
   4.9

==> Outputs/VOSL_QE.tex <==
-126.5

==> Outputs/VOSL_QE11.tex <==
-150.8

==> Outputs/VOSL_QE12.tex <==
   6.7

==> Outputs/VOSL_QE15.tex <==
   4.5

==> Outputs/VOSL_QE16.tex <==
   4.5

==> Outputs/VOSL_wo.tex <==
  17.1

==> Outputs/VOSL_wo15.tex <==
  17.1

==> Outputs/VOSL_wo_QE16.tex <==
  18.2
